Emergence of Hierarchy in Networked Endorsement Dynamics

Many social and biological systems are characterized by enduring hierarchies, including those organized around prestige in academia, dominance in animal groups, and desirability in online dating. Despite their ubiquity, the general mechanisms that explain the creation and endurance of such hierarchies are not well understood. We introduce a generative model for the dynamics of hierarchies using time-varying networks in which new links are formed based on the preferences of nodes in the current network and old links are forgotten over time. The model produces a range of hierarchical structures, ranging from egalitarianism to bistable hierarchies, and we derive critical points that separate these regimes in the limit of long system memory. Importantly, our model supports statistical inference, allowing for a principled comparison of generative mechanisms using data. We apply the model to study hierarchical structures in empirical data on hiring patterns among mathematicians, dominance relations among parakeets, and friendships among members of a fraternity, observing several persistent patterns as well as interpretable differences in the generative mechanisms favored by each. Our work contributes to the growing literature on statistically grounded models of time-varying networks.

==> assets/criticality_table.tex <==

    
\begin{tabular}{l l l l l}
                        &                 &  Root-Degree     &   PageRank      &  SpringRank    \\ 
    \toprule
    Math PhD            & $\beta_1^c$ &  \textbf{1.36}     &   1.18   &  2.00   \\ 	
    Exchange            & $\hat{\beta}_1$   &  \textbf{1.28}$_*$ (0.02)     &   0.74$_*$ (0.01)   &  2.99* (0.04)   \\ 
    \midrule
    Parakeets (G1)      & $\beta_1^c$ &  0.55      &  1.18     &  \textbf{2.00}    \\ 	
                        & $\hat{\beta}_1$   &  0.84$^*$ (0.05)     &  1.82$^*$ (0.08)    &  \textbf{3.03}$^*$ (0.16)   \\ 
    \midrule 
    Parakeets (G2)        & $\beta_1^c$ &  0.49      &  1.18     &  \textbf{2.00}    \\ 	
                           & $\hat{\beta}_1$ &  0.62$^*$ (0.03)     &  0.82$_*$ (0.04)    &  \textbf{2.86}$^*$ (0.14)   \\ 
    \midrule 
    Newcomb             & $\beta_1^c$ &  0.89      &  1.18    &  \textbf{2.00}    \\ 	
    Fraternity          & $\hat{\beta}_1$ &  0.95 (0.05)     &  1.21 (0.07)    &  \textbf{2.33}$^*$ (0.14)   \\ 
    \midrule
    % & \multicolumn{4}{l}{$^*$All parameters shown are nonzero with $p < 0.01$.} 
\end{tabular}

==> assets/inference_table.tex <==

    
\begin{tabular}{l l r r r}
                        &                 &  Root-Degree     &   PageRank      &  SpringRank    \\ 
    \toprule
    Math PhD            & $\hat{\lambda}$ &  0.87 (0.01)     &   0.96 (0.01)   &  0.91 (0.01)   \\ 	
    Exchange            & $\hat{\beta}_1$ &  1.28 (0.02)     &   0.74 (0.01)   &  2.99 (0.04)   \\ 
    (\emph{N} = 6,019)  & $\hat{\beta}_2$ & -0.18 (0.01)     &  -0.07 (0.00)   & -1.12 (0.04)   \\ 
    \cmidrule{2-5}
                        & $\mathcal{L}$   & \textbf{-14,379} & -15,001         & -14,927        \\
    \midrule
    Parakeets (G1)      & $\hat{\lambda}$ &  0.97 (0.08)     &  0.59 (0.08)    &  0.67 (0.14)   \\ 	
    (\emph{N} = 838)    & $\hat{\beta}_1$ &  0.84 (0.05)     &  1.82 (0.08)    &  3.03 (0.16)   \\ 
                        & $\hat{\beta}_2$ & -0.12 (0.01)     & -0.50 (0.03)    & -1.74 (0.12)   \\ 
    \cmidrule{2-5}
                        & $\mathcal{L}$   & -1,106           & -1,053          & \textbf{-964}  \\
    \midrule 
    Parakeets (G2)      & $\hat{\lambda}$ &  0.42 (0.07)     &  0.13 (0.03)    &  0.40 (0.06)   \\ 	
    (\emph{N} = 961)    & $\hat{\beta}_1$ &  0.62 (0.03)     &  0.82 (0.04)    &  2.86 (0.14)   \\ 
                        & $\hat{\beta}_2$ & -0.06 (0.01)     & -0.12 (0.01)    & -1.46 (0.12)   \\ 
    \cmidrule{2-5}
                        & $\mathcal{L}$   & -975             & -1029           & \textbf{-924}  \\
    \midrule 
    Newcomb             & $\hat{\lambda}$ &  0.56 (0.13)     &  0.81 (0.19)    &  0.71 (0.14)   \\ 	
    Fraternity          & $\hat{\beta}_1$ &  0.95 (0.05)     &  1.21 (0.07)    &  2.33 (0.14)   \\ 
    (\emph{N} = 1,428)  & $\hat{\beta}_2$ & -0.08 (0.03)     & -0.25 (0.05)    & -0.86 (0.16)   \\ 
    \cmidrule{2-5}
                        & $\mathcal{L}$   & -1,850           & -1,865          & \textbf{-1,841}\\
    \midrule
    % & \multicolumn{4}{l}{$^*$All parameters shown are nonzero with $p < 0.01$.} 
\end{tabular}

==> dgleich-extra.tex <==
\usepackage{ushort}
\newcommand{\cel}[1]{\ushort{#1}}
\newcommand{\cbmat}[1]{\left\{ \begin{matrix} #1 \end{matrix} \right\}}
\newcommand{\csbmat}[1]{\left\{\! \begin{smallmatrix} #1
\end{smallmatrix} \! \right\}}
%\newcommand{\csbmat}[1]{\underline{\sbmat{#1}}}
\newcommand{\smallmath}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\celm}[1]{\cel{\mat{#1}}}
\newcommand{\celv}[1]{\cel{\vec{#1}}}



\newcommand{\calpha}{\ensuremath{\cel{\alpha}}}
\newcommand{\cbeta}{\ensuremath{\cel{\beta}}}
\newcommand{\clambda}{\ensuremath{\cel{\lambda}}}

\newcommand{\cone}{\ensuremath{\cel{1}}}
\newcommand{\ca}{\ensuremath{\cel{a}}}
\newcommand{\cb}{\ensuremath{\cel{b}}}
\newcommand{\cc}{\ensuremath{\cel{c}}}
\newcommand{\cd}{\ensuremath{\cel{d}}}
\newcommand{\ce}{\ensuremath{\cel{e}}}
\newcommand{\cf}{\ensuremath{\cel{f}}}
\newcommand{\cg}{\ensuremath{\cel{g}}}
\newcommand{\ch}{\ensuremath{\cel{h}}}
\newcommand{\ci}{\ensuremath{\cel{i}}}
\newcommand{\cj}{\ensuremath{\cel{j}}}
\newcommand{\ck}{\ensuremath{\cel{k}}}
\newcommand{\cl}{\ensuremath{\cel{l}}}
\newcommand{\cm}{\ensuremath{\cel{m}}}
\newcommand{\cn}{\ensuremath{\cel{n}}}
\newcommand{\co}{\ensuremath{\cel{o}}}
\newcommand{\cp}{\ensuremath{\cel{p}}}
\newcommand{\cq}{\ensuremath{\cel{q}}}
%\newcommand{\cr}{\ensuremath{\cel{r}}}
\newcommand{\cs}{\ensuremath{\cel{s}}}
\newcommand{\ct}{\ensuremath{\cel{t}}}
\newcommand{\cu}{\ensuremath{\cel{u}}}
\newcommand{\cv}{\ensuremath{\cel{v}}}
\newcommand{\cw}{\ensuremath{\cel{w}}}
\newcommand{\cx}{\ensuremath{\cel{x}}}
\newcommand{\cy}{\ensuremath{\cel{y}}}
\newcommand{\cz}{\ensuremath{\cel{z}}}


\newcommand{\cA}{\ensuremath{\cel{A}}}
\newcommand{\cB}{\ensuremath{\cel{B}}}
\newcommand{\cC}{\ensuremath{\cel{C}}}
\newcommand{\cD}{\ensuremath{\cel{D}}}
\newcommand{\cE}{\ensuremath{\cel{E}}}
\newcommand{\cF}{\ensuremath{\cel{F}}}
\newcommand{\cG}{\ensuremath{\cel{G}}}
\newcommand{\cH}{\ensuremath{\cel{H}}}
\newcommand{\cI}{\ensuremath{\cel{I}}}
\newcommand{\cJ}{\ensuremath{\cel{J}}}
\newcommand{\cK}{\ensuremath{\cel{K}}}
\newcommand{\cL}{\ensuremath{\cel{L}}}
\newcommand{\cM}{\ensuremath{\cel{M}}}
\newcommand{\cN}{\ensuremath{\cel{N}}}
\newcommand{\cO}{\ensuremath{\cel{O}}}
\newcommand{\cP}{\ensuremath{\cel{P}}}
\newcommand{\cQ}{\ensuremath{\cel{Q}}}
\newcommand{\cR}{\ensuremath{\cel{R}}}
\newcommand{\cS}{\ensuremath{\cel{S}}}
\newcommand{\cT}{\ensuremath{\cel{T}}}
\newcommand{\cU}{\ensuremath{\cel{U}}}
\newcommand{\cV}{\ensuremath{\cel{V}}}
\newcommand{\cW}{\ensuremath{\cel{W}}}
\newcommand{\cX}{\ensuremath{\cel{X}}}
\newcommand{\cY}{\ensuremath{\cel{Y}}}
\newcommand{\cZ}{\ensuremath{\cel{Z}}}


\newcommand{\cva}{\ensuremath{\celv{a}}}
\newcommand{\cvb}{\ensuremath{\celv{b}}}
\newcommand{\cvc}{\ensuremath{\celv{c}}}
\newcommand{\cvd}{\ensuremath{\celv{d}}}
\newcommand{\cve}{\ensuremath{\celv{e}}}
\newcommand{\cvf}{\ensuremath{\celv{f}}}
\newcommand{\cvg}{\ensuremath{\celv{g}}}
\newcommand{\cvh}{\ensuremath{\celv{h}}}
\newcommand{\cvi}{\ensuremath{\celv{i}}}
\newcommand{\cvj}{\ensuremath{\celv{j}}}
\newcommand{\cvk}{\ensuremath{\celv{k}}}
\newcommand{\cvl}{\ensuremath{\celv{l}}}
\newcommand{\cvm}{\ensuremath{\celv{m}}}
\newcommand{\cvn}{\ensuremath{\celv{n}}}
\newcommand{\cvo}{\ensuremath{\celv{o}}}
\newcommand{\cvp}{\ensuremath{\celv{p}}}
\newcommand{\cvq}{\ensuremath{\celv{q}}}
\newcommand{\cvr}{\ensuremath{\celv{r}}}
\newcommand{\cvs}{\ensuremath{\celv{s}}}
\newcommand{\cvt}{\ensuremath{\celv{t}}}
\newcommand{\cvu}{\ensuremath{\celv{u}}}
\newcommand{\cvv}{\ensuremath{\celv{v}}}
\newcommand{\cvw}{\ensuremath{\celv{w}}}
\newcommand{\cvx}{\ensuremath{\celv{x}}}
\newcommand{\cvy}{\ensuremath{\celv{y}}}
\newcommand{\cvz}{\ensuremath{\celv{z}}}

\providecommand{\cmA}{\ensuremath{\celm{A}}}
\providecommand{\cmB}{\ensuremath{\celm{B}}}
\providecommand{\cmC}{\ensuremath{\celm{C}}}
\providecommand{\cmD}{\ensuremath{\celm{D}}}
\providecommand{\cmE}{\ensuremath{\celm{E}}}
\providecommand{\cmF}{\ensuremath{\celm{F}}}
\providecommand{\cmG}{\ensuremath{\celm{G}}}
\providecommand{\cmH}{\ensuremath{\celm{H}}}
\providecommand{\cmI}{\ensuremath{\celm{I}}}
\providecommand{\cmJ}{\ensuremath{\celm{J}}}
\providecommand{\cmK}{\ensuremath{\celm{K}}}
\providecommand{\cmL}{\ensuremath{\celm{L}}}
\providecommand{\cmM}{\ensuremath{\celm{M}}}
\providecommand{\cmN}{\ensuremath{\celm{N}}}
\providecommand{\cmO}{\ensuremath{\celm{O}}}
\providecommand{\cmP}{\ensuremath{\celm{P}}}
\providecommand{\cmQ}{\ensuremath{\celm{Q}}}
\providecommand{\cmR}{\ensuremath{\celm{R}}}
\providecommand{\cmS}{\ensuremath{\celm{S}}}
\providecommand{\cmT}{\ensuremath{\celm{T}}}
\providecommand{\cmU}{\ensuremath{\celm{U}}}
\providecommand{\cmV}{\ensuremath{\celm{V}}}
\providecommand{\cmW}{\ensuremath{\celm{W}}}
\providecommand{\cmX}{\ensuremath{\celm{X}}}
\providecommand{\cmY}{\ensuremath{\celm{Y}}}
\providecommand{\cmZ}{\ensuremath{\celm{Z}}}

\newcommand{\cmPt}{\cel{\mat{\tilde{P}}}}
\renewcommand{\cmPt}{\mat{\tilde{P}}}

\newcommand{\elm}[1]{\cel{#1}}

==> macros.tex <==
% New commands defined by Nicole.
% matrices
\newcommand{\mA}[0]{\mathbf{A}}
\newcommand{\mD}[0]{\mathbf{D}}
\newcommand{\mI}[0]{\mathbf{I}}
\newcommand{\mL}[0]{\mathbf{L}}
\newcommand{\mE}[0]{\mathbf{E}}
\newcommand{\mG}[0]{\mathbf{G}}
\newcommand{\mP}[0]{\mathbf{P}}
\newcommand{\mJ}[0]{\mathbf{J}}

\newcommand{\mGamma}[0]{\bm{\Gamma}}
\newcommand{\mSigma}[0]{\bm{\Sigma}}
\newcommand{\mDelta}[0]{\bm{\Delta}}
\newcommand{\mLambda}[0]{\bm{\Lambda}}

% for notational consistency, the boldface versions look kind of gross for some reason. 
\newcommand{\mPhi}[0]{\Phi} 
\newcommand{\mPsi}[0]{\Psi}

\newcommand{\mF}[0]{\mathbf{F}}
\newcommand{\mB}[0]{\mathbf{B}}
\newcommand{\mC}[0]{\mathbf{C}}
\newcommand{\mS}[0]{\mathbf{S}}
\newcommand{\mH}[0]{\mathbf{H}}
\newcommand{\mX}[0]{\mathbf{X}}
\newcommand{\mY}[0]{\mathbf{Y}}
\newcommand{\mM}[0]{\mathbf{M}}
\newcommand{\mR}[0]{\mathbf{R}}

% vectors
\newcommand{\vs}[0]{\mathbf{s}}
\newcommand{\vv}[0]{\mathbf{v}}
\newcommand{\vx}[0]{\mathbf{x}}
\newcommand{\vgamma}[0]{\bm{\gamma}}
\newcommand{\vphi}[0]{\bm{\phi}}
\newcommand{\ve}[0]{\mathbf{e}}
\newcommand{\vu}[0]{\mathbf{u}}
\newcommand{\diag}[1]{\textnormal{diag} #1}
\newcommand{\vf}[0]{\mathbf{f}}
\newcommand{\vh}[0]{\mathbf{h}}
\newcommand{\vk}[0]{\mathbf{k}}
\newcommand{\vzero}[0]{\mathbf{0}}
\newcommand{\vbeta}[0]{\bm{\beta}}
\newcommand{\vr}[0]{\mathbf{r}}
\newcommand{\vd}[0]{\mathbf{d}}
\newcommand{\vg}[0]{\mathbf{g}}
\newcommand{\vq}[0]{\mathbf{q}}

% sets
\newcommand{\cB}[0]{\mathcal{B}}
\newcommand{\cE}[0]{\mathcal{E}}

% fancy functions
\newcommand{\cL}[0]{\mathcal{L}}

% time indices
\renewcommand{\t}[0]{{(t)}}
\newcommand{\tplusone}[0]{{(t+1)}}
\newcommand{\tminusone}[0]{{(t-1)}}

% derivatives
\newcommand{\dds}[1]{\frac{\partial #1}{\partial \vs}}


% theorem environments

\newtheorem{thm}{Theorem}

\newtheorem{conj}{Conjecture}
\newtheorem{lm}{Lemma}
\newtheorem{cor}{Corrolary}
\newtheorem{clm}{Claim}
\newtheorem{dfn}{Definition}

\newtheorem{lemma}{Lemma}
\newtheorem{lemma*}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{prop*}{Proposition}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

% misc

\newcommand\abs[1]{\left|#1\right|}
\newcommand\E[0]{\mathbb{E}}
\newcommand\R[0]{\mathbb{R}}
\newcommand\decision[2]{\underset{#2}{\overset{#1}{\gtreqless}}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand\prob[0]{\mathbb{P}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\trace}[1]{\textnormal{tr}\left(#1\right)}
\newcommand{\var}[1]{\textnormal{var}\left(#1\right)}
\newcommand{\cov}[1]{\textnormal{cov}\left(#1\right)}
\newcommand{\innerprod}[1]{\langle #1 \rangle}
\newcommand{\bracket}[1]{\langle #1 \rangle}

% cleveref names
\crefname{thm}{Theorem}{Theorems}
\Crefname{thm}{Theorem}{Theorems}
% Dan comment: NO PURIST LEMMATA PLURALIZATION? ;D 
\crefname{lm}{Lemma}{Lemmas}
\Crefname{lm}{Lemma}{Lemmata}

\Crefname{clm}{Claim}{Claims}
\crefname{clm}{Claim}{Claims}

\Crefname{cor}{Corollary}{Corollaries}
\crefname{cor}{Corollary}{Corollaries}

\crefname{example}{example}{examples}
\Crefname{example}{Example}{Examples}
\Crefname{table}{Table}{Tables}

% Test
\Crefname{equation}{Equation}{Equations}
\crefname{equation}{Eq.\!}{Eqs.\!}
\Crefname{figure}{Figure}{Figures}
\crefname{figure}{Fig.\!}{Figs.\!}

% markup
\newcommand{\pc}[1]{
    \iftoggle{comments}{{\textcolor{blue}{[PHIL: #1]}}}{}%
}
\newcommand{\dan}[1]{
	\iftoggle{comments}{\textcolor{magenta}{#1}}{}% 
}
\newcommand{\mari}[1]{
	\iftoggle{comments}{\hspace{-6pt}
	{\textcolor{orange}{[MK: #1]}}}{}%
}
\newcommand{\nicole}[1]{
	\iftoggle{comments}{{\textcolor{olive}{#1}}}{}% 
}

\newcommand{\rev}[1]{\textcolor{blue}{#1}}

==> pnas-revision2/01_significance_statement_rev2.tex <==
Hierarchies structure the lives of many social animals, including humans. 
We propose a novel, generative model of time-varying networks in which endorsements between individuals give rise to enduring hierarchies.
For several network-based ranking functions, our model possesses a distinct, analytically tractable critical transition between egalitarian and hierarchical states. 
We also use our model to explore hierarchical structures in empirical data on hiring patterns among mathematicians, dominance relations among parakeets, and friendships among members of a fraternity, observing several persistent patterns.
Overall, our model enables data-informed modeling of hierarchical networks in social and biological systems. 

